DynOMo: Online Point Tracking by Dynamic Online Monocular Gaussian Reconstruction

Reconstructing scenes and tracking motion are two sides of the same coin. Tracking points allow for geometric reconstruction [14], while geometric reconstruction of (dynamic) scenes allows for 3D tracking of points over time [24, 39]. The latter was recently also exploited for 2D point tracking to overcome occlusion ambiguities by lifting tracking directly into 3D [38]. However, above approaches either require offline processing or multi-view camera setups both unrealistic for real-world applications like robot navigation or mixed reality. We target the challenge of online 2D and 3D point tracking from unposed monocular camera input introducing Dynamic Online Monocular Reconstruction (DynOMo). We leverage 3D Gaussian splatting to reconstruct dynamic scenes in an online fashion. Our approach extends 3D Gaussians to capture new content and object motions while estimating camera movements from a single RGB frame. DynOMo stands out by enabling emergence of point trajectories through robust image feature reconstruction and a novel similarity-enhanced regularization term, without requiring any correspondence-level supervision. It sets the first baseline for online point tracking with monocular unposed cameras, achieving performance on par with existing methods. We aim to inspire the community to advance online point tracking and reconstruction, expanding the applicability to diverse real-world scenarios.

==> sec/3_preliminaries.tex <==
% \section{3D Gaussians as Particles in 3D Space}
\section{Preliminary}
%\qj{@Jenny, I removed the $-\Sigma_i^{-1}$ to $\Sigma_{i}^{-1}$ in eq1, eq2 since I believe it was a typo.}
\label{sec:prel}

\PAR{3D Guassian Splatting.} 3D Gaussian Splatting (3DGS) \cite{kerbl3Dgaussians} represents the appearance and geometry of 
% the underlying 3D world 
a 3D scene with a set of $M$ explicit anisotropic 3D Gaussian distributions $\mathcal{G} = \{G_i\}_{i=0}^M$. Each 3D Gaussian is parametrized by its mean $\mu_i$ and covariance matrix $\Sigma_i$ and defined as:

\begin{equation}
    % G_i(x; \mu_i, \Sigma_i) = e^{-\frac{1}{2}(x-\mu_i)^T-\Sigma_i^{-1}(x-\mu_i)}.
    G_i(x; \mu_i, \Sigma_i) = e^{-\frac{1}{2}(x-\mu_i)^T\Sigma_i^{-1}(x-\mu_i)}.
\end{equation}
The covariance matrix is defined as $\Sigma_i = R_is_is_i^TR_i^T$ where $s_i$ is  a scale vector and $R_i$ a rotation matrix defined by a quaternion vector $q_i$. 
Each $G_i$ additionally is assigned a color $c_i$ and opacity $o_i$ attributes. 
% 
% 
% Given camera extrinsics $E_c$ and intrinsics $I_c$, 
To efficiently render a RGB image at a given camera, the 3D Gaussians are splatted into 2D Gaussians $G_{i, 2D}(p;\mu_{i, 2D}, \Sigma_{i, 2D})$ on the image plane utilizing an affine approximation of the exact projection \cite{Zwicker2001VolumeSplatting}. 
Finally, the color of a pixel $p$ is computed by $\alpha$-composing the color values of the projected 2D Gaussians 
% $\{G_{i, 2D}\}_{i \in H}$ 
that intersect with pixel $p$:
\begin{equation}
    C_p = \sum_{i \in H} T_i \alpha_i c_i
\end{equation}
% where $\alpha_i = o_i e^{-\frac{1}{2}(p-\mu_{i,2D})^T-\Sigma_{i,2D}^{-1}(p-\mu_{i,2D})}$ 
where $\alpha_i = o_i e^{-\frac{1}{2}(p-\mu_{i,2D})^T\Sigma_{i,2D}^{-1}(p-\mu_{i,2D})}$ 
and $T_i = \prod_{j=1}^{i-1} (1-\alpha_j)$. 
% 
The splatting-based rendering process is fully differentiable thus the parameters $(\mu_i, q_i, s_i, c_i, i_o)$ can be 
optimized directly via computing an image reconstruction loss
\begin{equation}
    \mathcal{L}_I=||I-\hat{I}||_1
    \label{eq:im_rec_loss}
\end{equation}
between a training image $I$ and the synthesized image $\hat{I}$ rendered at that training camera pose.

% are optimized in an offline way and over multiple views of the scene using an image reconstruction loss. For example, $l_I=||I-\hat{I}||_1$ is commonly used where $\hat{I}$ is a training image from the input sequence and $I$ the rendered image given the pixel colors $C_p$. 

% \PAR{Dynamic 3D Gaussian Splatting.}
% To model dynamic scenes, recent works introduced deformation fields \cite{duisterhof2023MDSplat,li2023spacetime,wu20234dgaussians,yang2023deformable3dgs,yang2023gs4d,sun20243dgstream} or motion basis vectors \cite{kratimenos2024dynmf,som2024shapeofmotion}. We follow \cite{luiten2023dynamic} that first initializes a point cloud at time step 0 given a mutli-camera setup with known camera poses. Then the gaussians positions are updated utilizing a view reconstruction loss as well as 3D rigidity, rotation, and isometry losses. The latter enforce a Gaussian and its k nearest neighbors to move rigidly, have the same rotation and the keep their initial distance in the 3D space, respectively. Those assumptions hold even for non-rigid objects when applied only in a local window. All loss functions are weighted by the distance between two gaussians in the 3D space. Please refer to the supplementary material for detailed equations.

% \qj{Talk about the definition of Dynamic 3D GS, like how it works.}



% The explicit representation of 3DGS allows to view each $G_i$ as a volume, \ie, a particle in the 3D space. Hence, a reconstruction can be seen as a composition of particles in 3D space. 
% Different from static scene reconstruction, in dynamic scenes the Gaussian particles can move over time. However, just optimizing using image reconstruction losses does not necessarily lead to physically sound motion of the Gaussians or correct motion reconstruction. 
% The 2D image can be explained by different motions of the Gaussians in the 3D space, especially if they are of similar color. Hence, the motion and position of Gaussians is ambiguous - Gaussians can cheat. 
% %
% To this end, \cite{luiten2023dynamic} introduced physics-based regularization priors, namely a 3D rigidity, rotation, and isometry loss. The losses enforce a Gaussian and its k nearest neighbors (kNN) to move rigidly, have the same rotation and the keep their initial distance in the 3D space, respectively. Those assumptions hold even for non-rigid objects when applied over the local kNN set. All loss functions are weighted by the distance between two gaussians in the 3D space. Please refer to the supplementary material for detailed equations.

% We build on the loss functions introduced in \cite{luiten2023dynamic} and adapt them for our monocular setting where the above mentioned challenges are even enforced.




\PAR{Dynamic 3D Gaussian Splatting.} 
The vanilla 3DGS assumes the scene is static. Our work adopts the formulation of D-3DGS~\cite{luiten2023dynamic} to model a dynamic scene with 3D Gaussians by keeping a set of 3D Gaussian parameters per timestamp.
As the image reconstruction loss $\mathcal{L}_I$ can not fully constrain the motions of the Gaussians in 3D, they introduce three regularization losses, \ie, short-term local-rigidity loss $\mathcal{L}^{rigid}$, local-rotation similarity loss $\mathcal{L}^{rot}$ and a long-term local-isometry loss $\mathcal{L}^{iso}$, to regularize the optimization procedure to be physically plausible. Due to the space limit, we provide the equations for those losses in the supplymentary material.
% 
While those losses work well for their multi-camera setting, we show necessary adaptation (\cf \cref{subsec:motion_regularizer}) is required when switching to monocular camera setting.

\PAR{Online 3DGS SLAM.}
SplaTAM~\cite{keetha2024splatam} exploits 3DGS for SLAM in static scenes with the following pipeline.
They start by initializing a set of Gaussians at time step $t=0$ given ground truth depth maps. 
At each new timestamp, they 
(i) track cameras by optimizing the camera pose based on image and depth reconstruction losses; 
(ii) add new Gaussians for unobserved regions based on a densification mask $M_D(p)$ computed by applying a threshold on pixel densities, \ie, 
\begin{equation}
    M_D(p) = (\sum_{i \in H} T_i \alpha_i) < 0.5,
    \label{eq:densification}
\end{equation}
(iii) update the Gaussians by the same losses in (i);
(iv) initialize the next timestamp camera pose by a constant velocity forward projection.
%
Our method (\cf \cref{sec:method}) builds on top of this pipeline and extend it with dynamic 3DGS for handling dynamic scenes.




% \PAR{Online Monocular Reconstruction Pipeline.}
% The explicit representation of 3DGS allows to view each $G_i$ as a volume, \ie, a particle in the 3D space. Hence, a reconstruction can be seen as a composition of particles in 3D space.

% \cite{keetha2024splatam} exploits this fact for online reconstruction in the SLAM application. 

% They start by initializing a set of Gaussians $\mathcal{G}$ by $\mathcal{G}^0 = \{G^0_i\}$ at time step $t=0$ given ground truth depth maps. 
% At each time step $t=\tau$ they (i) update the camera position $\mathcal{C}_{\tau}$; 
% (ii) add new Gaussians $\mathcal{G} \leftarrow \mathcal{G} \cup \mathcal{G}^{\tau}$ for unobserved regions using the densification concept. This means Gaussians are only added where the image space is not densely covered

% \begin{equation}
%     M_D(p) = (\sum_{i \in H} T_i \alpha_i) < 0.5
% \end{equation}

% where $p$ is a given pixel; (iii) update the parameters of the Gaussians; (iv) forward propagate $\mathcal{C}_{\tau}$ to the next time step $t=\tau+1$ given their prior motion.
% %
% While we follow a similar pipeline, we adapted the pipeline in order to be applicable to dynamic scenes as we will introduce in \cref{sec:method}.




==> tabs/supp_jono.tex <==
\begin{table*}[!thp]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{4.2pt}
    %\resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc}
    \toprule
        %& \multicolumn{6}{c}{\textit{3DIoU}}\\
        Method & $MTE_{2D}$ $\downarrow$ & $S_{2D}$ $\uparrow$ & $\delta_{avg, 2D}$ $\uparrow$ & \%1 & \%8 & \%16 & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$ \\
        \midrule
        \midrule
        D-3DGS \cite{luiten2023dynamic} & 10.5 & 76.8 & 57.4 & 20.6 & 75.9 & 82.5 & 33.2 & 0.96 & 0.05 \\
        D-3DGS-M & 23.3 & 41.0 & 30.6& 14.8 & 37.9 & 47.5  & \textbf{39.6}  & \textbf{0.98} & \textbf{0.03} \\
        D-3DGS-M$_f$ & 29.5 & 43.5 & 28.3 & 9.7 & 38.7 & 46.3  & 37.8 & 0.97 & 0.06 \\
        \midrule
        \method-DA \cite{Yang2024depthanything} & \textbf{3.7} & 83.7 & 59.0 & 19.6 & 80.3 & 88.7 & 32.5 & 0.96 & 0.90 \\
        % \method (D-3DGS-D) & 9.3 & 73.8 & 52.7 & 31.6 & 0.96 & 0.10 & & \\
        \method-D-3DGS-D & 6.3 & \textbf{85.7} & \textbf{61.8} & \textbf{25.3} & \textbf{83.6} & \textbf{90.3} & 31.9 & 0.96 & 0.09 \\
        \method-S-D-3DGS-D  \textcolor{red}{incomplete} & 8.1 &  73.1 & 47.0 & 1.0 & 69.0 & 82.3 & 27.1 & 0.89 & 0.21 \\
        % \method (DepthAnything) & 7.6 & 68.4 & 53.4  & 19.2 & 69.5 & 67.3  & 32.1 & 0.96 & 0.11\\
        % \method-D-3DGS-PC & 26.7 & 54.6 & 36.4  & 11.3 & 51.3 & 59.8 & 37.6 & 0.99 & 0.05 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison on Panoptic Studio \cite{luiten2023dynamic} for 2D Point Tracking:} We compare our performance on the updated setting explained in \cref{subsec:dataset}. D-3DGS-M is \cite{luiten2023dynamic} optimized using a single camera. In D-3DGS-M$_f$ we reduce the number of iterations during optimization. We observe that despite our approach only has access to one single view, our 2D point tracking outperforms the one obtained by \cite{luiten2023dynamic}. Note that since we optimize for point tracking rather than novel-view synthesis, we report rendering metrics on training views. Hence, that this is just for reference not for SOTA comparisons.}
    %}
    \label{tab:jono2d}
\end{table*}


\begin{table}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{4.2pt}
    %\resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|ccc}
    \toprule
        %& \multicolumn{6}{c}{\textit{3DIoU}}\\
        Method & $MTE_{3D}$ $\downarrow$ & $S_{3D}$ $\uparrow$ & $\delta_{avg, 3D}$ $\uparrow$ \\
        \midrule
        \midrule
        D-3DGS \cite{luiten2023dynamic} & 13.7 & 86.8 & 43.7 \\
        D-3DGS-M & 56.0 & 44.5 & 7.3  \\
        D-3DGS-M$_f$ & 50.5 & 43.9 & 6.6  \\
        \midrule
         \method-DA \cite{Yang2024depthanything} & 70.7 & 25.4 & 0.7 \\  % not_higher_lr_original_size_transformed from 3D
        % \method-D-3DGS-PC & 31.1 & 71.2 & 11.7  \\ % not_higher_lr_normal_size_jono_pc_orig_size from 3D
        \method-D-3DGS-D & 26.1 & 73.0 & 12.7  \\ % not_higher_lr_orig_size_transformed_jono_depth from 3D
        % \method (DepthAnything) & 147.7 & 0.0 & 0.3  \\ % not_higher_lr_original_size_transformed
       \method-S-D-3DGS-D \textcolor{red}{incomplete} & 31.6 & 62.0 & 10.0 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison on Panoptic Studio \cite{luiten2023dynamic} for 3D Point Tracking:} We compare our performance to on 3D trajectories. D-3DGS-M is \cite{luiten2023dynamic} optimized using a single camera. In D-3DGS-M$_f$ we reduce the number of iterations during optimization. We observe that $MTE_{3D}$ and $\delta_{avg, 3D}$ are considerably lower than D-3DGS. However, our performance significantly ourperforms the monocular setup of \cite{luiten2023dynamic} D-3DGS-M. This shows that our optimization indeed enforces Gaussiam particles to move appropirately in the 3D space.}
    %}
    \label{tab:jono3d}
\end{table}

